A note on the Nielsen realization problem for connected sums of $S^2 \times S^1$

We consider finite group-actions on 3-manifolds $\cal H_g$ obtained as the connected sum of $g$ copies of $S^2 \times S^1$, with free fundamental group $F_g$ of rank $g$. We prove that, for $g > 1$, a finite group of diffeomorphisms of $\cal H_g$ inducing a trivial action on homology is cyclic. As a consequence, no non-cyclic subgroup of the twist subgroup of the mapping class group of $\cal H_g$ (generated by Dehn twists along embedded 2-spheres) can be realized by diffeomorphisms (in the sense of the Nielsen realization problem). We also discuss when a finite subgroup of the outer automorphism group ${\rm Out}(F_g)$ of the fundamental group of $\cal H_g$ can be realized by a group of diffeomorphisms of $\cal H_g$.

==> Erratum <==

\input amssym.def
\input amssym
\magnification=1200
\parindent0pt
\hsize=16 true cm
\baselineskip=13  pt plus .2pt
$ $


\def\G{(\Gamma,{\cal G})}
\def\Z{{\Bbb Z}}
\def\D{{\Bbb D}}
\def\A{{\Bbb A}}
\def\S{{\Bbb S}}
\def\H{{\cal H}}



{\bf Erratum to:}

\medskip

{\bf A note on the Nielsen realization problem}
{\bf for  connected sums of $S^2  \times S^1$}



\bigskip 


Bruno P. Zimmermann 

\smallskip

Department of Mathematics,  University of Trieste, Italy


\bigskip   \bigskip


In the recent paper [1], we considered the Nielsen realization problem for finite
subgroups of the mapping class groups ${\rm Mod}(\H_g)$ of the 3-manifolds 
$\H_g = \sharp_g (S^2 \times S^1)$ obtained as the connected sums of $g$ copies of $S^2
\times S^1$ (called {\it closed handles of genus $g$} in [1]).  
Denoting by ${\rm Twist}(\H_g)$ the subgroup of ${\rm Mod}(\H_g)$ generated
by all Dehn twists along embedded 2-spheres in $\H_g$, there is a short exact sequence

$$ 1  \to  {\rm Twist}(\H_g)  \hookrightarrow {\rm Mod}(\H_g) \to  {\rm
Out}(\pi_1(\H_g)) \to 1,$$

and ${\rm Twist}(\H_g) \cong  (\Bbb Z_2)^g$ is generated by the 
twists around non-seperating 2-spheres in $\H_g$. 
As a consequence of the main theorem, it is claimed in [1] that no non-trivial element of
the twist group 
${\rm Twist}(\H_g)$ can be realized (represented) by a periodic diffeomorphism of $\H_g$
(in the sense of the Nielsen realization problem); the proof
of the main theorem in [1] is incomplete and the theorem has to be modified as follows.


\bigskip


{\bf Theorem.}  {\sl  Let $G$ be a finite group of orientation-preserving diffeomorphisms
of a closed handle
$\H_g$ of genus $g > 1$. If $G$ induces the trivial action on the first homology of
$\H_g$ then $G$ is a cyclic group.} 


\bigskip


It is further claimed in [1] that $G$ is a subgroup of an $S^1$-action on $\H_g$ 
but the proof is incomplete since, in general, the various $S^1$-actions on the building
blocks  (0-handles) of $\H_g$ don't fit together along the 1-handles to define an
$S^1$-action on all of $\H_g$.


\bigskip


{\bf Corollary.}  {\sl  A non-cyclic subgroup of the 
twist group  ${\rm Twist}(\H_g)$ cannot be realized by diffeomorphisms of
$\H_g$.}


\bigskip


It is a consequence of the main theorem in a recent preprint by Lei Chen and Bena
Tshishiku [2] that cyclic subgroups of ${\rm Twist}(\H_g)$ can be realized by
diffeomorphisms; more generally, the authors show that, for every closed oriented
3-manifold $M$ which is a connected sum, a subgroup $G$ of the twist group can be realized
if and only if $G$ is cyclic and $M$ is a connected sum of lens spaces (including $S^2
\times S^1$).


\bigskip  \bigskip
\vfill \eject

\centerline {\bf References}


\medskip


\item {[1]}  Bruno Zimmermann, {\it  A note on the Nielsen realization problem for
connected sums of $S^2 \times S^1$,} Rend. Istit. Mat. Univ. Trieste 53,  2021

(electronic versions in:  rendiconti.dmi.units.it,  arXiv:2105.04901)


\medskip


\item {[2]}  Lei Chen, Bena Tshishiku, {\it Nielsen realization for twists on
3-manifolds,}  preprint 2022  (arXiv:2204.04820)





\bye








